Pricing service maintenance contracts using predictive analytics

As more manufacturers shift their focus from selling products to end solutions, full-service maintenance contracts gain traction in the business world. These contracts cover all maintenance related costs during a predetermined horizon in exchange for a fixed service fee and relieve customers from uncertain maintenance costs. To guarantee profitability, the service fees should at least cover the expected costs during the contract horizon. As these expected costs may depend on several machine-dependent characteristics, e.g. operational environment, the service fees should also be differentiated based on these characteristics. If not, customers that are less prone to high maintenance costs will not buy into or renege on the contract. The latter can lead to adverse selection and leave the service provider with a maintenance-heavy portfolio, which may be detrimental to the profitability of the service contracts. We contribute to the literature with a data-driven tariff plan based on the calibration of predictive models that take into account the different machine profiles. This conveys to the service provider which machine profiles should be attracted at which price. We demonstrate the advantage of a differentiated tariff plan and show how it better protects against adverse selection.

==> calibration.tex <==
\section{Calibration of predictive models for pricing}
\label{sec: calibration}
Once the dataset of failure and maintenance events is available, we calibrate predictive models to the event data capturing the failure occurrences, failure types, failure and maintenance costs observed over the machine-specific timelines. 
We hereby identify the impact of the machine-dependent characteristics $\bm{x}_1$ and $\bm{x}_2(t)$ to determine a machine-dependent technical (break-even) price $P^\star|\bm{x}_1,\bm{x}_2(t)$.

\subsection{Likelihoods of the predictive models}
We propose a hierarchical approach inspired by \citet{frees2008hierarchical} and decompose the joint probability distribution of the event data in its stochastic elements: failure times and types, failure and maintenance costs. 
The event timeline of a single machine is defined by the set of all events registered on the same machine in the dataset, see Table \ref{tab: sim data}.
The joint probability distribution of the timeline of a single machine with failure times $\bm{T}$, failure types $\bm{Y}$, failure costs $\bm{X}$ and maintenance costs $\bm{S}$ is $f(\boldsymbol{T},\boldsymbol{Y},\boldsymbol{X},\boldsymbol{S})$, can be decomposed as follows:
\begin{equation}
	f(\boldsymbol{T},\boldsymbol{Y},\boldsymbol{X},\boldsymbol{S})= f(\boldsymbol{T},\bm{Y})\cdot f(\boldsymbol{X}\vert \boldsymbol{T},\boldsymbol{Y})\cdot f(\boldsymbol{S}\vert \boldsymbol{T},\boldsymbol{Y},\bm{X}),
\end{equation}
where covariates are omitted to promote legibility.
%Alternatively, a contract time-line can be interpreted in a more granular way by considering the total number of failures $N$ during the contract duration $\Delta t$ instead of accounting for all specific failure times.
%In this case the total probability distribution takes the form $f(N, \Delta t, \boldsymbol{Y},\boldsymbol{X},\boldsymbol{S})$ and can be decomposed in similar fashion as
%\begin{equation}
%	f(N, e, \boldsymbol{Y},\boldsymbol{X},\boldsymbol{S})= f(N\vert \Delta t) \cdot f(\boldsymbol{Y}\vert N)  \cdot f(\boldsymbol{X}\vert \boldsymbol{T},\boldsymbol{Y})\cdot f(\boldsymbol{S}).
%\end{equation}
%Although this approach takes into account less detailed, it is more straightforward to implement.


\paragraph{Time-to-failure likelihood}
The first component $f(\bm{T},\bm{Y})$ deals with the failures times and types.
First, we analyze the failure times, while only distinguishing between minor and catastrophic failures.
To price full-service maintenance contracts, it is not necessary to know the exact failure times, it suffices to estimate the number of failures during the contract period, see Equation \eqref{eq: breakeven P}.
This gives us two possible approaches to model the data on occurrences of failures as observed over the lifetime of a machine or service contract. 
On the one hand we can propose and calibrate a time-to-failure model which uses the full detail of the failure times, as displayed in Table \ref{tab: sim data}.
Such a model does not only allow for the assessment of the number of failures during the contract horizon, but also the prediction of the failure times.
On the other hand, aggregating the time-to-failure data into discrete time periods allows the use of count models. 
Such regression models predict the number of failures in a next time period.
In line with the granularity of our simulation, we opt for time-to-failure models as they provide more detail than count models. 

To calibrate the time-to-failure model, we maximize its specific time-to-event log-likelihood.
Each failure~$j$ in the dataset is characterized by a vector $(y_j,t_j,t_{0,j},c_j)$, where \\ $y_{j}\in \{\text{minor},\text{catastrophic}\}$ is the failure type, $t_j$ indicates the failure time, $t_{0,j}$ the time of the previous failure and $c_j \in \{0,1\}$, with $0$ indicating censoring of the event.
In first instance we aggregate the different minor failure types as a single type.
This mimics the simulation, where the minor failure types are generated in a second stage.
The log-likelihood $\mathcal{L}(\alpha_{\lambda_0},\kappa_{\lambda_0},\gamma_{\lambda_0},\bm{\beta}_1,\bm{\beta}_2,\alpha_{c},\kappa_{c})$ then becomes
\begin{equation}
\mathcal{L}(\alpha_{\lambda_0},\kappa_{\lambda_0},\gamma_{\lambda_0},\bm{\beta}_1,\bm{\beta}_2,\alpha_{c},\kappa_{c}) =\sum_{j} \left[c_j\log(\lambda_{y_{j}}(t_j)) + \log(S_T(t_j\vert t_{0,j}))\right],
\label{eq: lik}
\end{equation}
where $j$ runs over all observed failures, registered on all machines in the portfolio, over the historical observation period. 
$S_T(t\vert t_0)$ is the survival function for the time-to-next-failure, see Equation \eqref{eq: total surv function} and $\lambda_{y_{j}}(t)$ is the type-specific \colg{failure intensity function}, see Equations \eqref{eq: minor failure hazard} and \eqref{eq: imperfect hazard}, and \eqref{eq: weibull hazard} for minor and catastrophic failures respectively.
Maximizing the log-likelihood $\mathcal{L}(\alpha_{\lambda_0},\kappa_{\lambda_0},\gamma_{\lambda_0},\bm{\beta}_1,\bm{\beta}_2,\alpha_{c},\kappa_{c})$ gives estimates for the model parameters, i.e. $\alpha_{\lambda_0},\kappa_{\lambda_0}$ and $\gamma_{\lambda_0}$ for the baseline hazard, $\bm{\beta}_1$ and $\bm{\beta}_2$ for the influence of the machine covariates, and $\alpha_{c}$ and $\kappa_{c}$ for the catastrophic failures.

\paragraph{Likelihood for minor failure types}
The component $f(\bm{T},\bm{Y})$ also embodies the failure types.
Previously, we incorporated only the distinction between minor and catastrophic failures.
Now we handle the minor failure types.
We estimate the parameters of the multinomial logit model which delivers the probabilities for the minor failure types $Y\vert (Y\in \mathcal{N}_{f,\text{minor}})$ \citep{frees2008hierarchical}.
Each minor failure $j$ is characterized by an observed failure type $y_{j}$.
Using the observed data the log-likelihood $\mathcal{L}(\{\bm{\alpha}_y\vert y \in \mathcal{N}_{f,\text{minor}}\})$ for a dataset with failures $j$, registered on all machines in the portfolio, is 
\begin{equation}
	\mathcal{L}(\{\bm{\alpha}_y\vert y \in \mathcal{N}_{f,\text{minor}}\}) = \sum_{j} \log \left(\Pr[Y = y_{j}\vert Y\in \mathcal{N}_{f,\text{minor}}]\right).
	\label{eq: logit lik}
\end{equation} 
Equation \eqref{eq: multinom prob} gives an explicit expression for $\Pr[Y = y_{j}\vert Y\in \mathcal{N}_{f,\text{minor}}]$.
Maximizing the log-likelihood $\mathcal{L}(\{\bm{\alpha}_y\vert y \in \mathcal{N}_{f,\text{minor}}\})$ gives estimates for the parameters $\bm{\alpha}_y$ driving each minor failure type $y\ (\in \{1,.., n_{f,\text{minor}}\})$.\footnote{In the R \citep{Rsoftware} package \textquoteleft nnet\textquoteright\ \citep{nnet} maximum likelihood estimation for the multinomial logit model is available.}

\paragraph{Severity likelihood}
The last two components of the decomposition $f(\boldsymbol{X}\vert \boldsymbol{T},\boldsymbol{Y})$ and \\
$f(\boldsymbol{S}\vert\boldsymbol{T},\boldsymbol{Y}, \boldsymbol{X})$ deal with the failure and maintenance costs respectively.
We calibrate the parameters in the distributional model making use of distributions for the costs on the one hand and a copula for the dependency of costs in case of co-occurring failures on the other hand. 
The log-likelihood $\mathcal{L}(\bm{\gamma})$ for a dataset with maintenance actions $j$ and associated costs $s_j$, registered on all machines in the portfolio, is
\begin{equation}
	\mathcal{L}(\bm{\gamma}) = \sum_{j} \log\left(f_S(s_j)\right),
	\label{eq costs lik}
\end{equation}
where $f_S(s)$ is the probability density function associated with the maintenance costs, see Equation \eqref{eq: costs distr}. 
Maximizing the log-likelihood $\mathcal{L}(\bm{\gamma})$ gives estimates for $\bm{\gamma}$.
Similarly, estimates for $\bm{\gamma}_{y}\ (\forall y \in \mathcal{N}_{f,\text{minor}})$ and $\bm{\gamma}_c$ can be found.
In our experiments, we use a gamma distribution for the costs and a Frank copula\footnote{In the R \citep{Rsoftware} package \textquoteleft copula\textquoteright\ \citep{copula2,copula3,copula4,copula1} maximum likelihood estimation for the Frank copula is available.} for the dependency between costs of co-occurring failures \citep{frees2008hierarchical}.

\vspace{5mm}
\noindent
In Appendix~\ref{appendix verification} we provide the results of an extensive simulation study, where we generate multiple portfolios of machines over time (along the recipe in Section \ref{sec: simulation model}) and calibrate the proposed hierarchical likelihood on each of these simulated datasets. 
%Note that the calibrated parameters for our generated datasets should be reasonably close to our simulation parameters.
Appendix~\ref{appendix verification} reveals that our calibration strategy is capable of retrieving the parameter values used when simulating the different datasets.

\subsection{From predictive models to pricing}
Based on the calibrated predictive models, the break-even price $P^\star$ in Equations \eqref{eq: breakeven P} and \eqref{eq: cond break even price}, can now be determined.
We make this explicit by reformulating the break-even price in function of the predictive models, taking into account the risk factors $\bm{\chi_1},\bm{w},\bm{w}_y,\bm{w}_c \subseteq \bm{x_1}$, and $\bm{\chi_2}(t)\subseteq \bm{x_2}(t)$:
\begin{equation}
\begin{aligned}
P^\star&\vert \bm{\chi_1},\bm{\chi_2}(t),\bm{w},\bm{w}_y,\bm{w}_c=E[N_{f,c}\vert\bm{\chi}_1,\bm{\chi}_2(t)]\cdot E[X_{c}\vert \boldsymbol{w}_c] \\ &+E[N_{f,\text{minor}}\vert \bm{\chi}_1,\bm{\chi}_2(t)] \cdot \sum_{y = 1}^{n_{f,\text{minor}}}\Pr[Y=y \vert Y\in \mathcal{N}_{f,\text{minor}} ,\bm{z}]\cdot E[X_{y}\vert \boldsymbol{w}_y]\\ &+  n_{m} \cdot E[S\vert \boldsymbol{w}],
\end{aligned}	
\label{eq: price (pricing)}
\end{equation}
where $E[N_{f,\text{minor}}\vert\bm{\chi}_1,\bm{\chi}_2(t)]$ is the predicted number of minor failures within the contract duration and $E[N_{f,c}\vert \bm{\chi}_1,\bm{\chi}_2(t)]$ the predicted number of catastrophic failures for machine characteristics $\bm{\chi}_1$ and $\bm{\chi}_2(t)$, obtained from the predictive time-to-failure models with likelihood given in Equation~\eqref{eq: lik}.
Remark that the explicit dependence of the price on the contract duration is omitted from Equation \eqref{eq: price (pricing)}, however it is evident that its components are dependent on the contract duration.
As the break-even price depends on the machine characteristics, different tariff plans are generated depending on the set of characteristics that are included in the predictive models.

We opt for Monte Carlo simulation to estimate the different terms in Equation~\eqref{eq: price (pricing)}.
The generated paths rely on the simulation engine described in Section~\ref{simulation}, where the input parameters for the simulation are the parameters resulting from the calibration of the predictive models.
Next to an estimate for the expected values in Equation~\eqref{eq: price (pricing)}, other risk measures could be estimated from the generated scenarios. 
This allows to estimate a risk margin on top of the break-even price, as well as more detailed risk assessment of the contracts in the portfolio.

==> tikz_workflow.tex <==
\begin{tikzpicture}[align=center, auto, scale=0.4, every node/.style={scale=0.45}]
	% color
	\definecolor{dark_magenta}{RGB}{222, 89, 113}
	\definecolor{grey}{RGB}{128,128,128}
	% coordinates
	\coordinate (simulation) at (0,1.5);
	\coordinate (calibration) at (9,1.5);
	\coordinate (pricing) at (18,1.5);
	\coordinate (evaluation) at (27,1.5);
	
	% titles
	\node at (simulation) {\Large{\textbf{Simulation engine}}};
	\node at (calibration) {\Large{\textbf{Calibration}}};
	\node at (pricing) {\Large{\textbf{Pricing}}};
	\node at (evaluation) {\Large{\textbf{Economic evaluation}}};
	
	\node at (0,0.75) {\large{\textbf{Section 4}}};
	\node at (9,0.75) {\large{\textbf{Sections 5 \& 6}}};
	\node at (18,0.75) {\large{\textbf{Sections 5 \& 6}}};
	\node at (27,0.75) {\large{\textbf{Section 7}}};
	
	\node at (4.5,-8) {\large{\textbf{Generated data sets}}};
	\node at (13.5,5) {\large{\textbf{Calibrated parameters}}};
	\node at (22.5,-8) {\large{\textbf{tariff plans}}};
	
	% big rectangles
	\draw [rounded corners] (-3.5,2) rectangle (3.5, -7) {};
	\draw [rounded corners] (5.5,2) rectangle (12.5, -7) {};
	\draw [rounded corners] (14.5,2) rectangle (21.5, -7) {};
	\draw [rounded corners] (23.5,2) rectangle (30.5, -7) {};
	
	% small rectangles
	\draw [rounded corners] (1.5,-7.5) rectangle (7.5, -10.5) {};
	\draw [rounded corners] (10.5,2.5) rectangle (16.5, 5.5) {};
	\draw [rounded corners] (19.5,-7.5) rectangle (25.5, -10.5) {};
	
	% lines
	\draw [](0,-7) -- (0,-9);
	\draw [->] (0,-9) -- (1.5,-9);
	\draw [](7.5,-9) -- (9,-9);
	\draw [->] (9,-9) -- (9,-7);
	
	\draw [](9,2) -- (9,4);
	\draw [->] (9,4) -- (10.5,4);
	\draw [](16.5,4) -- (18,4);
	\draw [->] (18,4) -- (18,2);
	
	\draw [](18,-7) -- (18,-9);
	\draw [->] (18,-9) -- (19.5,-9);
	\draw [](25.5,-9) -- (27,-9);
	\draw [->] (27,-9) -- (27,-7);
	
	% Simulation
	\node [block_small] (init) at (0,-.5){generate population};
	\node [block_small] (frequency) at (0,-2.25){generate failure times};
	\node [block_small] (type)at (0,-4){generate failure types};
	\node [block_small] (severity) at (0,-5.75) {generate costs};
	\path [line] (init) -- (frequency);
	\path [line] (frequency) -- (type);
	\path [line] (type) -- (severity);
	
	% Calibration 
	\node [block_small] (cal 4) at (9,-.5){time-to-failure model};
	\node [block_small] (cal 2) at (9,-3){multinomial model};
	\node [block_small] (cal 3)at (9,-5.5){costs models};
	\path [line] (cal 2) -- (cal 3);
	\path [line] (cal 4) -- (cal 2);
	
	% Pricing
	\node [block_small] (price 1) at (18,-.5){ variable selection};
	\node [block_small] (price 2) at (18,-3){model selection};
	\node [block_small] (price 3) at (18,-5.5){determine price};	
	\path [line] (price 1) -- (price 2);
	\path [line] (price 2) -- (price 1);
	\path [line] (price 2) -- (price 3);
	
	% Evaluation
	\node [block_small] (value 1) at (27,-.5){in- and out-of-sample};
	\node [block_small] (value 2) at (27,-3){loss ratio};
	\node [block_small] (value 4) at (27,-5.5){quantile plot, Lorenz curves and Gini index};
	\path [line] (value 1) -- (value 2);
	\path [line] (value 2) -- (value 4);
	
	% Datasets
	\node at (3,-8.5) {data 1};
	\draw [rounded corners] (2,-8.25) rectangle (4, -10.25) {};
	\draw (2.5,-8.75) -- (2.5,-10.25);
	\draw (3,-8.75) -- (3,-10.25);
	\draw (3.5,-8.75) -- (3.5,-10.25);
	\draw (2,-8.75) -- (4,-8.75);
	\draw (2,-9) -- (4,-9);
	\draw (2,-9.75) -- (4,-9.75);
	\draw (2,-9.5) -- (4,-9.5);
	\draw (2,-10) -- (4,-10);
	\draw (2,-9.25) -- (4,-9.25);
	\node at (5.25,-8.5) {data 2};
	\draw [rounded corners] (4.25,-8.25) rectangle (6.25, -10.25) {};
	\draw (4.75,-8.75) -- (4.75,-10.25);
	\draw (5.25,-8.75) -- (5.25,-10.25);
	\draw (5.75,-8.75) -- (5.75,-10.25);
	\draw (4.25,-8.75) -- (6.25,-8.75);
	\draw (4.25,-9) -- (6.25,-9);
	\draw (4.25,-9.75) -- (6.25,-9.75);
	\draw (4.25,-9.5) -- (6.25,-9.5);
	\draw (4.25,-10) -- (6.25,-10);
	\draw (4.25,-9.25) -- (6.25,-9.25);
	\node [right] at (6.25,-9.25) {\textbf{\dots}};
	
	% Calibr param
	\node at (13.5,4) {\LARGE{$\alpha,\bm{\beta},\bm{\gamma}$}};
	
	% Pricing schemes
	\node at (22.5,-9) {\LARGE{$P^\star_a, P^\star_b, P^\star_c$}};
\end{tikzpicture}
